Restoring Hebrew Diacritics Without a Dictionary

We demonstrate that it is feasible to diacritize Hebrew script without any human-curated resources other than plain diacritized text. We present NAKDIMON, a two-layer character level LSTM, that performs on par with much more complicated curation-dependent systems, across a diverse array of modern Hebrew sources.

==> tab_ablations.tex <==

% For new table:
% =============
% Nakdimon_0
% Nakdimon (full -- same one as in test table)
% 1 layer (h=400)
% 1 layer (h=557, |params| like in full)
% 2 layers, h=200
% 3 layers (h=400)
% no scheduling (best lr of 3e-4, 1e-3, 2e-3)
% training on modern only
% something with the way the losses are aggregated?


\begin{table}
    \centering
    \small
    \begin{tabular}{lcccc} \toprule
        Components & \textsc{dec} & \textsc{cha} & \textsc{wor} & \textsc{voc} \\
        \midrule
        \textit{Dicta (reference)} & \textit{98.09} & \textit{96.72}  & \textit{91.56} & \textit{94.33} \\
        Full ($l=2, h=400$) & 97.19 & 95.06 & 85.74 & 89.95 \\
        \midrule
        \phantom{Full (}$l=2, h=600$ & 97.22 & 95.10 & 85.92 & 90.11 \\
        \phantom{Full (}$l=1, h=400$ & 95.53 & 92.23 & 76.80 & 82.64 \\
        \phantom{Full (}$l=1, h=557$ & 95.62 & 92.37 & 77.30 & 83.01 \\
        \phantom{Full (}$LR=3\cdot 10^{-3}$ & 96.79 & 94.36 & 83.26 & 88.05 \\
        \midrule
        \phantom{Full (}\textsc{modern} only & 95.95 & 92.88 & 79.95 & 84.77 \\
        \phantom{Full (}Pre-trained LM & 97.19 & 95.07 & 85.81 & 90.06 \\
        \bottomrule
    \end{tabular}
    \caption{Ablation results (macro \% accuracy) for \sysname{} variants on a validation set (40 docs, 27,681 tokens).}
    \label{tab:abl}
\end{table}


==> tab_examples.tex <==
\begin{table}[]
    \centering
    \begin{tabular}{lc} \toprule
        % \cjRL{d*:bAriyM +sErA.siytiy lOmAr} \\
        % \cjRL{dbryM /sr.syty lwmr} \\ \bottomrule
        \multirow{3}{*}{(a)} & \cjRL{qnyty 'tmwl mknsyym lbnym} \\
        & \sffamily{\small kaniti etmol mixnasayim ????} \\
        & `I bought (unspecified) yesterday' \\
        \multirow{3}{*}{(b)} & \cjRL{qAniytiy 'Et:mOl mik:nAsayiym l:bAniym}  \\
        & \sffamily{\small kaniti etmol mixnasayim levanim} \\
        & `I bought white trousers yesterday' \\
        \multirow{3}{*}{(c)} & \cjRL{qAniytiy 'Et:mOl mik:nAsayiym lab*Aniym}  \\
        & \sffamily{\small kaniti etmol mixnasayim la-banim} \\
        & `I bought trousers for the boys yesterday' \\ \bottomrule
    \end{tabular}
    \caption{An example of an undotted Hebrew text (a) (written right to left) which can be interpreted in at least two different ways (b,c), dotted and pronounced differently, both meaningful and reasonable.
    % Disambiguation is impossible without long-range context or extralinguistic knowledge.
    }% \todo{Figure out font issues: \url{http://texdoc.net/texmf-dist/doc/latex/babel/babel.pdf}; or just insert a .png.}}
    \label{tab:ex}
\end{table}

